Examining the behaviour of state-of-the-art convolutional neural networks for brain tumor detection with and without transfer learning

Distinguishing normal from malignant and determining the tumor type are critical components of brain tumor diagnosis. Two different kinds of dataset are investigated using state-of-the-art CNN models in this research work. One dataset(binary) has images of normal and tumor types, while another(multi-class) provides all images of tumors classified as glioma, meningioma, or pituitary. The experiments were conducted in these dataset with transfer learning from pre-trained weights from ImageNet as well as initializing the weights randomly. The experimental environment is equivalent for all models in this study in order to make a fair comparison. For both of the dataset, the validation set are same for all the models where train data is 60% while the rest is 40% for validation. With the proposed techniques in this research, the EfficientNet-B5 architecture outperforms all the state-of-the-art models in the binary-classification dataset with the accuracy of 99.75% and 98.61% accuracy for the multi-class dataset. This research also demonstrates the behaviour of convergence of validation loss in different weight initialization techniques.

==> elsevierGuide.tex <==
%! Author = sbbfti
%! Date = 10/06/2020

\section{The Elsevier article class}

\paragraph{Installation} If the document class \emph{elsarticle} is not available on your computer, you can download and install the system package \emph{texlive-publishers} (Linux) or install the \LaTeX\ package \emph{elsarticle} using the package manager of your \TeX\ installation, which is typically \TeX\ Live or Mik\TeX.

\paragraph{Usage} Once the package is properly installed, you can use the document class \emph{elsarticle} to create a manuscript. Please make sure that your manuscript follows the guidelines in the Guide for Authors of the relevant journal. It is not necessary to typeset your manuscript in exactly the same way as an article, unless you are submitting to a camera-ready copy (CRC) journal.

\paragraph{Functionality} The Elsevier article class is based on the standard article class and supports almost all of the functionality of that class. In addition, it features commands and options to format the
\begin{itemize}
\item document style
\item baselineskip
\item front matter
\item keywords and MSC codes
\item theorems, definitions and proofs
\item lables of enumerations
\item citation style and labeling.
\end{itemize}

\section{Front matter}

The author names and affiliations could be formatted in two ways:
\begin{enumerate}[(1)]
\item Group the authors per affiliation.
\item Use footnotes to indicate the affiliations.
\end{enumerate}
See the front matter of this document for examples. You are recommended to conform your choice to the journal you are submitting to.

\section{Bibliography styles}

There are various bibliography styles available. You can select the style of your choice in the preamble of this document. These styles are Elsevier styles based on standard styles like Harvard and Vancouver. Please use Bib\TeX\ to generate your bibliography and include DOIs whenever available.

Here are two sample references: \cite{Feynman1963118,Dirac1953888}.

==> introduction.tex <==
%! Author = sbbfti
%! Date = 10/06/2020

% Document

\section{Introduction}
Brain tumour one of the most deadliest kinds of disease which is caused for abnormal growth of of abnormal cells that have formed in the brain. Some brain tumors are cancerous (malignant), while others are not (non-malignant). Since the brain is the control 
center of the human body, developing tumors can put pressure 
on the skull and cause negative human health \cite{1}. The number 
of deaths due to brain tumors are increasing day by day. 
Theciteore, early diagnosis is important for all brain tumors, as 
in all diseases. Early diagnosis of brain tumor is often made by 
magnetic resonance imaging (MRI) \cite{2}.

Appropriate diagnosis of a brain tumor is critical for appropriate treatment planning and patient care. Manual classification of brain tumor MR images with similar structures or appearances is a complex and time-consuming task that is contingent on the radiologist's availability and experience in identifying and classifying the brain tumor. The radiologist classifies brain tumors in two ways: I determining if the brain MR pictures are normal or abnormal. (ii) Classify aberrant brain magnetic resonance pictures into distinct tumor categories. Such manual classification of brain tumors is impracticable, nonreproducible, and time consuming when dealing with vast amounts of MRI data. To address this issue, automatic classification may be used to classify MR images of brain tumors with minimal interaction from radiologists.

Accurate and timely diagnosis of brain tumors is critical for effective treatment. The treatment modality chosen is determined by the stage of the tumor at the time of diagnosis, its pathological kind, and grade. Numerous ways have computer-aided diagnostic (CAD) approaches assisted neuro-oncologists. In neuro-oncology, CAD applications include tumor identification, classification, and grading. Brain tumor classification using CAD is a well-researched area.\cite{3}. Grading glioma, a significant subtype of malignant tumor, is another area of research in this arena.\cite{4}. The aforementioned computer-aided design (CAD) systems rely on brain magnetic resonance imaging (MRI) images. This is because MRI pictures have a larger contrast for soft tissues in the brain than computed tomography (CT) images provide.

Classification approaches based on traditional machine learning typically involve many steps, including preprocessing, feature extraction, feature selection, dimension reduction, and classification. Typically, feature extraction is dependent on the expert's topic expertise. It is difficult for a non-expert to do research using typical machine learning approaches. Traditional machine learning relies heavily on feature extraction, and classification accuracy is highly dependent on the extracted features. Two types of feature extraction exist. The first category includes low-level (global) characteristics such as intensity and texture. First- and second-order statistics (e.g., mean, standard deviation, and skewness) obtained from the gray level co-occurrence matrix (GLMC), shape, wavelet transform, and Gabor feature.





==> myacronyms.tex <==
%! Author = sbbfti
%! Date = 10/06/2020

\newacronym{ti}{$T_{i}$}{indoor air temperature, $^{\circ}$C}
\newacronym{tout}{$T_{out}$}{outdoor air temperature, $^{\circ}$C}
\newacronym{top}{$T_{o}$}{operative air temperature}
\newacronym{ts}{$T_{s}$}{supply air temperature, $^{\circ}$C}
\newacronym{v}{$\dot{V}$}{measured volumetric flow rate, L/s}
\newacronym{vsp}{$\dot{V}_{sp}$}{volumetric flow rate set-point, L/s}
\newacronym{tsph}{$T_{sp,h}$}{heating zone temperature set-point, $^{\circ}$C}
\newacronym{tspc}{$T_{sp,c}$}{cooling zone temperature set-point}
\newacronym{ghi}{$G_{hi}$}{global horizontal irradiance, W/m$^2$}
\newacronym{BMS}{BMS}{Building Management System}
\newacronym{pmv}{PMV}{Predicted Mean Vote}
\newacronym{HVAC}{HVAC}{Heating, Ventilation, and Air Conditioning}
\newacronym{VAV}{VAV}{Variable Air Volume}
\newacronym{AHU}{AHU}{Air Handling Unit}

==> results.tex <==
%! Author = sbbfti
%! Date = 10/06/2020


\section{Results}

The results of the experiment are shown in Figure \ref{fig:cbe_ashrae}.

$ x^n + y^n = z^n $







\begin{center}
\begin{table*}
\centering
\caption{Binary Classification With Transfer Learning}\label{Tab1}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Model Name       & Accuracy & F1-Score & Precision & Recall   & Loss   \\
\hline
ResNet-50        & 0.990833 & 0.989277 & 0.990278  & 0.991437 & 0.060031 \\
\hline
ResNet18         & 0.994167 & 0.993184 & 0.994500  & 0.994413 & 0.034172 \\
\hline
ResNext50        & 0.995833 & 0.995123 & 0.995444  & 0.996246 & 0.016570 \\
\hline
GoogleNet        & 0.995000 & 0.992858 & 0.993389  & 0.994111 & 0.020670 \\
\hline
Efficient Net b0 & 0.995833 & 0.995521 & 0.996722  & 0.995690 & 0.016866 \\
\hline
Efficient Net b1 & 0.996667 & 0.995123 & 0.995611  & 0.996357 & 0.010314 \\
\hline
Efficient Net b2 & 0.995833 & 0.995123 & 0.995889  & 0.996079 & 0.014472 \\
\hline
Efficient Net b3 & 0.996667 & 0.996491 & 0.997111  & 0.996722 & 0.016532 \\
\hline
Efficient Net b4 & 0.996667 & 0.996367 & 0.997389  & 0.996278 & 0.010307 \\
\hline
Efficient Net b5 & 0.997500 & 0.997460 & 0.997667  & 0.997833 & 0.012521 \\
\hline
Efficient Net b6 & 0.995833 & 0.995521 & 0.996556  & 0.995667 & 0.019978 \\
\hline
Efficient Net b7 & 0.996667 & 0.996244 & 0.996944  & 0.996556 & 0.020426 \\
\hline
   
\end{tabular}
\end{table*}

\end{center}

\begin{table*}[]
\centering
\caption{Binary Classification Without Transfer Learning}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Model Name       & Accuracy & F1-Score & Precision & Recall   & Loss     \\
\hline
ResNet-50        & 0.988333 & 0.986491 & 0.988056  & 0.989270 & 0.057198 \\
\hline
ResNet18         & 0.994167 & 0.989153 & 0.990333  & 0.991603 & 0.038533 \\
\hline
ResNext50        & 0.990833 & 0.989713 & 0.990778  & 0.991802 & 0.045017 \\
\hline
GoogleNet        & 0.990000 & 0.989226 & 0.990944  & 0.990389 & 0.041164 \\
\hline
Efficient Net b0 & 0.995833 & 0.995521 & 0.996722  & 0.996167 & 0.014202 \\
\hline
Efficient Net b1 & 0.997500 & 0.997337 & 0.997944  & 0.997389 & 0.015023 \\
\hline
Efficient Net b2 & 0.994167 & 0.993705 & 0.995167  & 0.994944 & 0.029045 \\
\hline
Efficient Net b3 & 0.996667 & 0.996491 & 0.997278  & 0.996556 & 0.012283 \\
\hline
Efficient Net b4 & 0.996667 & 0.996367 & 0.996667  & 0.997000 & 0.013449 \\
\hline
Efficient Net b5 & 0.996667 & 0.996367 & 0.997389  & 0.996278 & 0.010942 \\
\hline
Efficient Net b6 & 0.995000 & 0.994674 & 0.995500  & 0.995167 & 0.022722 \\
\hline
Efficient Net b7 & 0.995833 & 0.995000 & 0.995167  & 0.996357 & 0.018193 \\
\hline
                 
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{Multiclass Classification With Transfer Learning}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Model Name       & Accuracy & F1-Score & Precision & Recall   & Loss     \\
\hline
ResNet-50        & 0.988333 & 0.986491 & 0.988056  & 0.989270 & 0.057198 \\
\hline
ResNet18         & 0.994167 & 0.989153 & 0.990333  & 0.991603 & 0.038533 \\
\hline
ResNext50        & 0.990833 & 0.989713 & 0.990778  & 0.991802 & 0.045017 \\
\hline
GoogleNet        & 0.990000 & 0.989226 & 0.990944  & 0.990389 & 0.041164 \\
\hline
Efficient Net b0 & 0.995833 & 0.995521 & 0.996722  & 0.996167 & 0.014202 \\
\hline
Efficient Net b1 & 0.997500 & 0.997337 & 0.997944  & 0.997389 & 0.015023 \\
\hline
Efficient Net b2 & 0.994167 & 0.993705 & 0.995167  & 0.994944 & 0.029045 \\
\hline
Efficient Net b3 & 0.996667 & 0.996491 & 0.997278  & 0.996556 & 0.012283 \\
\hline
Efficient Net b4 & 0.996667 & 0.996367 & 0.996667  & 0.997000 & 0.013449 \\
\hline
Efficient Net b5 & 0.996667 & 0.996367 & 0.997389  & 0.996278 & 0.010942 \\
\hline
Efficient Net b6 & 0.995000 & 0.994674 & 0.995500  & 0.995167 & 0.022722 \\
\hline
Efficient Net b7 & 0.995833 & 0.995000 & 0.995167  & 0.996357 & 0.018193 \\
\hline    
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\caption{Multi-class Classification Without Transfer Learning}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Model Name       & Accuracy & F1-Score & Precision & Recall   & Loss     \\
\hline
ResNet-50        & 0.988333 & 0.986491 & 0.988056  & 0.989270 & 0.057198 \\
\hline
ResNet18         & 0.994167 & 0.989153 & 0.990333  & 0.991603 & 0.038533 \\
\hline
ResNext50        & 0.990833 & 0.989713 & 0.990778  & 0.991802 & 0.045017 \\
\hline
GoogleNet        & 0.990000 & 0.989226 & 0.990944  & 0.990389 & 0.041164 \\
\hline

Efficient Net b0 & 0.995833 & 0.995521 & 0.996722  & 0.996167 & 0.014202 \\
\hline
Efficient Net b1 & 0.997500 & 0.997337 & 0.997944  & 0.997389 & 0.015023 \\
\hline
Efficient Net b2 & 0.994167 & 0.993705 & 0.995167  & 0.994944 & 0.029045 \\
\hline
Efficient Net b3 & 0.996667 & 0.996491 & 0.997278  & 0.996556 & 0.012283 \\
\hline
Efficient Net b4 & 0.996667 & 0.996367 & 0.996667  & 0.997000 & 0.013449 \\
\hline
Efficient Net b5 & 0.996667 & 0.996367 & 0.997389  & 0.996278 & 0.010942 \\
\hline
Efficient Net b6 & 0.995000 & 0.994674 & 0.995500  & 0.995167 & 0.022722 \\
\hline
Efficient Net b7 & 0.995833 & 0.995000 & 0.995167  & 0.996357 & 0.018193 \\
\hline
\end{tabular}
\end{table*}



==> tbl_resp_speed.tex <==
\begin{tabular}{lrrr}
\toprule
  userid &  count &    mean &      std \\
\midrule
  dorn01 &  222.0 &   545.4 &   1710.2 \\
  dorn02 &  460.0 &    12.5 &     17.2 \\
  dorn03 &  412.0 &  1717.7 &   7317.2 \\
  dorn04 &  149.0 &   774.6 &   3143.2 \\
  dorn05 &  382.0 &   281.0 &   3608.4 \\
  dorn06 &  175.0 &   598.3 &   3499.2 \\
  dorn07 &  339.0 &  4010.5 &  66551.9 \\
  dorn08 &  381.0 &   820.2 &   4467.8 \\
  dorn09 &  350.0 &    15.8 &     88.2 \\
  dorn11 &  346.0 &   456.2 &   1842.6 \\
  dorn12 &  407.0 &   458.9 &   2838.2 \\
  dorn13 &  340.0 &   489.8 &   4290.0 \\
  dorn14 &  249.0 &  2528.1 &   7956.8 \\
  dorn15 &  351.0 &   141.4 &    595.0 \\
  dorn18 &  238.0 &   709.2 &   4298.4 \\
  dorn19 &   94.0 &    21.6 &     72.4 \\
  dorn20 &  248.0 &   663.0 &   3431.1 \\
 dorn999 &   69.0 &    70.7 &    306.2 \\
    test &   18.0 &     1.4 &      3.2 \\
\bottomrule
\end{tabular}


==> titleAbstract.tex <==
%! Author = sbbfti
%! Date = 10/06/2020

\begin{frontmatter}

\title{Examining the behaviour of state-of-the-art deep learning methodologies for Brain Tumor classification with and with-out transfer learning}
\tnotetext[mytitlenote]{Fully documented templates are available in the elsarticle package on \href{http://www.ctan.org/tex-archive/macros/latex/contrib/elsarticle}{CTAN}.}

%% Group authors per affiliation:
\author{Md. Atik Ahamed, Rabeya Tus Sadia}
\address{Dhaka, Bangladesh}
% \fntext[myfootnote]{Since 1880.}

%% or include affiliations in footnotes:
\author[mymainaddress,mysecondaryaddress]{Department of Computer Science \& Engineering}
\ead[url]{www.elsevier.com}

\author[mysecondaryaddress]{Global Customer Service\corref{mycorrespondingauthor}}
\cortext[mycorrespondingauthor]{Corresponding author}
\ead{support@elsevier.com}

\address[mymainaddress]{1600 John F Kennedy Boulevard, Philadelphia}
\address[mysecondaryaddress]{360 Park Avenue South, New York}

\begin{abstract}

\end{abstract}

\begin{keyword}
\texttt{elsarticle.cls}\sep \LaTeX\sep Elsevier \sep template
\MSC[2010] 00-01\sep  99-00
\end{keyword}

\end{frontmatter}

